System-Wide Security for Offline Payment Terminals

Most self-service payment terminals require network connectivity for processing electronic payments. The necessity to maintain network connectivity increases costs, introduces cybersecurity risks, and significantly limits the number of places where the terminals can be installed. Leading payment service providers have proposed offline payment solutions that rely on algorithmically generated payment tokens. Existing payment token solutions, however, require complex mechanisms for authentication, transaction management, and most importantly, security risk management. In this paper, we present VolgaPay, a blockchain-based system that allows merchants to deploy secure offline payment terminal infrastructure that does not require collection and storage of any sensitive data. We design a novel payment protocol which mitigates security threats for all the participants of VolgaPay, such that the maximum loss from gaining full access to any component by an adversary incurs only a limited scope of harm. We achieve significant enhancements in security, operation efficiency, and cost reduction via a combination of polynomial multi-hash chain micropayment channels and blockchain grafting for off-chain channel state transition. We implement the VolgaPay payment system, and with thorough evaluation and security analysis, we demonstrate that VolgaPay is capable of delivering a fast, secure, and cost-efficient solution for offline payment terminals.

==> discussion.tex <==

\section{Discussion}

The major practical challenge to commercial deployment of offline terminals based on \volgapay design is the need to use cryptocurrency for funding the public smart contract. Although major cryptocurrencies, such as Bitcoin or Ethereum, are very easy to purchase, store, and transact with, the world has not yet adjusted to them. Also, the market value of major cryptocurrencies is highly fluctuating, which might impair net profit estimation. The use of so-called tether coins, whose market value is bound to a certain classic currency, e.g., U.S. dollar, allows to partially address the challenge. However, the tether cryptocurrencies are still underrepresented in the market and under-researched by the expert community.

% Our fully-functional prototype demonstrates the feasibility of \volgapay, and thorough evaluation of delays, fees, communication overhead, and security threats demonstrates security and efficiency of the system proposed in this work. However, the usability, efficiency and security of \volgapay can be further improved, if necessary, if additional features, described below, are added to the system.

% \subsection{Duplex Channel for Refund}
% For the sake of simplicity, we desined the prototype of \volgapay using a simplex payment channel. Yet the design of a duplex channel, in which the merchant has the ability to refund the client, is also possible.

% \subsection{Merchant Hash Chain Seed Protection}
% Our prototype assumes that the Merchant infrastructure maintains access to the set of hash chain seeds for all clients all the time. We also assume that each redundancy server has copies of seeds for each smart contract.
